BASS: Block-wise Adaptation for Speech Summarization

End-to-end speech summarization has been shown to improve performance over cascade baselines. However, such models are difficult to train on very large inputs (dozens of minutes or hours) owing to compute restrictions and are hence trained with truncated model inputs. Truncation leads to poorer models, and a solution to this problem rests in block-wise modeling, i.e., processing a portion of the input frames at a time. In this paper, we develop a method that allows one to train summarization models on very long sequences in an incremental manner. Speech summarization is realized as a streaming process, where hypothesis summaries are updated every block based on new acoustic information. We devise and test strategies to pass semantic context across the blocks. Experiments on the How2 dataset demonstrate that the proposed block-wise training method improves by 3 points absolute on ROUGE-L over a truncated input baseline.

==> sections/results.tex <==

% \begin{table}[!ht]
% \caption{Performance of Truncated Speech Summarization models on 10-minute long test recordings across different features. Models are trained on 10-minute-long audio. R-1, R-2, R-3 represent the ROUGE-1, ROUGE-2, and ROUGE-L metrics respectively}
% \label{tab:acoustic_features_comparison}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{lrrrrr}
% \hline
% Input Feature   & R-1\uparrow   & R-2\uparrow & R-L\uparrow & METEOR\uparrow & BERTScore\uparrow \\ \hline
% HuBERT          & 19.60  & 4.26 & 13.61 & 10.25 & 80.98 \\ 
% WavLM           & 12.11 & 1.07 & 8.89 & 5.70 & 78.50   \\ 
% %Spectral**        & 21.52 & 4.59 & 15.19 & 10.05 & 82.81 \\
% Spectral        & 20.20 & 3.55 & 13.93 & 9.35 & 82.59 \\
% \hline
% \end{tabular}
% }
% \end{table}

\begin{table}[!ht]
\caption{Performance of BASS models with block level inference across different implementations of the semantic updater model. Models are pre-trained on 5 minutes and fine-tuned on 10 minutes. R-1, R-2, R-3 represent the ROUGE-1, ROUGE-2, and ROUGE-L metrics respectively}
\label{tab:updater_comparison}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lrrrrr}
    \toprule

Updater    & R-1\uparrow   & R-2\uparrow   & R-L\uparrow   & METEOR\uparrow & BERTScore\uparrow \\ 
\toprule
Concat     & 28.27 & 11.75 & 21.75 & 15.84  & 83.25     \\ 
Gated Attn & 26.15 & 11.22 & 20.49 & 13.80  & 83.52     \\ 
Hier. Attn & 26.11 & 10.50 & 19.50 & 13.30  & 83.40     \\ 
\bottomrule
\end{tabular}
}
\end{table}

\begin{table}[h]
    \centering
    \caption{Part-of-speech coverage between the Predicted Summary and the Reference for Truncated 5-minute baseline and BASS-ADAPT 10-minute model}
    \begin{tabular}{lrrrrr}
    \toprule
         Model & Noun & Verb & Adj & Adv & Prop.Noun \\
         \toprule
         Trunc 5-minute & 0.23 & 0.12 & 0.14 & 0.10 & 0.16 \\
        BASS-ADAPT & 0.40 & 0.27 & 0.28 & 0.33 & 0.171 \\
        \bottomrule
    \end{tabular}
    \label{tab:pos_analysis}
\end{table}

\section{Experimental Results}


% \subsection{Acoustic Features for Speech Summarization}

% Table \ref{tab:acoustic_features_comparison} compares self-supervised features for TED talk summarization and shows that HuBERT outperforms WavLM for the task of speech summarization. Therefore, HuBERT features are used for the remainder of our experiments. 

% Self-supervised features do improve performance on TED talk summarization, similar to other tasks like Speech Recognition and Spoken Language Understanding. 

\subsection{Truncated Input Baselines}
First, we train end-to-end summarization baseline models on truncated inputs (\texttt{Trunc}) that are 5 minutes long and 10 minutes long. We note 10 minutes is the longest we can use with the standard self-attention on our V100-32G GPU. Table \ref{tab:bass_result_summary} reports the results of training on truncated inputs and evaluating recordings that are 5 and 10 minutes long. We find that inference on longer recordings than used in training improves summarization performance slightly. 

%We also find that our reproduction of ~\cite{shon2022slueted} attains slightly lower performance with 10 minute recordings. 

\subsection{Block-wise Training versus Truncated Training}
The proposed BASS method can be used to help models trained on shorter recordings adapt to longer inputs (\texttt{BASS-Adapt}), or to train models from scratch in a block-wise manner (\texttt{BASS-Train}).
Inference for blockwise models can be performed in the \texttt{standard} manner, i.e., where the entire input is fed in at once to predict the final output. Alternatively, \texttt{Block} inference can be performed, where the input is fed as abutting blocks of input as described in Section \ref{section:blockwise_formulation}.   

We train \texttt{BASS-Adapt} initialized from the 5-minute truncated baseline to handle 10-minute recordings, and infer using \textbf{standard} and \texttt{block} mechanisms. \texttt{BASS-Adapt} is compared against \texttt{BASS-Train} by training a model on 10-minute-long recordings from scratch using our BASS algorithm. 

We compare both strategies for model adaptation and training in Table \ref{tab:bass_result_summary}. We see that the proposed \texttt{BASS-Adapt} approach outperforms \texttt{BASS-Train} on ROUGE and METEOR scores. We also observe that our proposed BASS algorithm improves over the truncated 5-minute baseline and also the truncated 10-minute baseline. \texttt{BASS-Adapt} with block inference results in a 5-point improvement in ROUGE-L over the best-truncated baseline. We also observe a 7-point improvement in ROUGE-L between the truncated baseline and the \texttt{BASS-Adapt} model with standard inference, suggesting that block-wise training helps the model derive potentially more accurate latent semantic representations. 

Finally, Table \ref{tab:pos_analysis} sheds light on the improvement in the prediction of different parts of speech in the reference summary using the best \texttt{BASS-ADAPT} model. We observe that the proposed model generally improves the prediction of all parts of speech but obtains small improvements on proper nouns. This demonstrates that end-to-end models find named 
entity prediction challenging, providing a direction for future work. 



% First, we train baseline models on truncated 5-minute and 10-minute long inputs. Then we use BASS to fine-tune the pre-trained 5-minute model on 10 minutes of audio. This is called the block-wise adapted model. We also use BASS to train a model on 10 minutes of audio from scratch and refer to this as the block-wise trained model. 



\subsection{Comparison of Block-wise Adaptation Strategies}

Table \ref{tab:updater_comparison} compares the various modeling strategies for the semantic updater. We observe that simply concatenating the semantic embedding of the previous (one) block with the current block yields significant improvements in summarization performance. \\




\noindent \textbf{Limitations}: One of the limitations of this work is that BASS requires strong pre-training on truncated inputs to obtain the best performance, along with larger than usual block sizes. For instance, using a few seconds of input for a block is likely insufficient to train a robust model. Attention-based sequence models are not very strong at identifying the correct output lengths ~\cite{deng22b_interspeech}, and this forms another limiting factor in model performance. 



==> sections/results.v2.tex <==

\begin{table}[!ht]
\caption{Performance of Truncated Speech Summarization models on 10-minute long test recordings across different features. Models are trained on 10-minute-long audio. R-1, R-2, R-3 represent the ROUGE-1, ROUGE-2, and ROUGE-L metrics respectively}
\label{tab:acoustic_features_comparison}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lrrrrr}
\hline
Input Feature   & R-1\uparrow   & R-2\uparrow & R-L\uparrow & METEOR\uparrow & BERTScore\uparrow \\ \hline
HuBERT          & 19.60  & 4.26 & 13.61 & 10.25 & 80.98 \\ 
WavLM           & 12.11 & 1.07 & 8.89 & 5.70 & 78.50   \\ 
Spectral        & 20.20 & 3.55 & 13.93 & 9.35 & 82.59 \\
\hline
\end{tabular}
}
\end{table}

\vspace{0.1}
% \begin{table}[h]
%     \centering
%     \caption{Part-of-speech coverage between the Predicted Summary and the Reference for Truncated 5-minute baseline and BASS-ADAPT 10-minute model}
%     \begin{tabular}{lrrrrr}
%     \toprule
%          Model & Noun & Verb & Adj & Adv & Prop.Noun \\
%          \toprule
%          Trunc 5-minute & 0.23 & 0.12 & 0.14 & 0.10 & 0.16 \\
%         BASS-ADAPT & 0.40 & 0.27 & 0.28 & 0.33 & 0.171 \\
%         \bottomrule
%     \end{tabular}
%     \label{tab:pos_analysis}
% \end{table}

\section{Experimental Results}


% \subsection{Acoustic Features for Speech Summarization}



% Self-supervised features do improve performance on TED talk summarization, similar to other tasks like Speech Recognition and Spoken Language Understanding. 

\subsection{Truncated Input Baselines}
Table \ref{tab:acoustic_features_comparison} compares acoustic features for TED talk summarization and shows that HuBERT outperforms WavLM, but performs slightly worse than spectral features. Therefore, spectral features are used for the remainder of our experiments. 
First, we train end-to-end summarization baseline models on truncated inputs (\texttt{Trunc}) that are 5 minutes long and 10 minutes long. We note 10 minutes is the longest we can use with the standard self-attention on our V100-32G GPU. Table \ref{tab:bass_result_summary} reports the results of training on truncated inputs and evaluating recordings that are 5 and 10 minutes long. We find that inference on longer recordings than used in training improves summarization performance slightly. 

%We also find that our reproduction of ~\cite{shon2022slueted} attains slightly lower performance with 10 minute recordings. 

\subsection{Block-wise Training versus Truncated Training}
The proposed BASS method can be used to help models trained on shorter recordings adapt to longer inputs (\texttt{BASS-Adapt}), or to train models from scratch in a block-wise manner (\texttt{BASS-Train}).
Inference for blockwise models can be performed in the \texttt{standard} manner, i.e., where the entire input is fed in at once to predict the final output. Alternatively, \texttt{Block} inference can be performed, where the input is fed as abutting blocks of input as described in Section \ref{section:blockwise_formulation}.   

We train \texttt{BASS-Adapt} initialized from the 5-minute truncated baseline to handle 10-minute recordings, and infer using \textbf{standard} and \texttt{block} mechanisms. \texttt{BASS-Adapt} is compared against \texttt{BASS-Train} by training a model on 10-minute-long recordings from scratch using our BASS algorithm. 

We compare both strategies for model adaptation and training in Table \ref{tab:bass_result_summary}. We see that the proposed \texttt{BASS-Adapt} approach outperforms \texttt{BASS-Train} on ROUGE and METEOR scores. We also observe that our proposed BASS algorithm improves over the truncated 5-minute baseline and also the truncated 10-minute baseline. \texttt{BASS-Adapt} with block inference results in a 5-point improvement in ROUGE-L over the best-truncated baseline. We also observe a 7-point improvement in ROUGE-L between the truncated baseline and the \texttt{BASS-Adapt} model with standard inference, suggesting that block-wise training helps the model derive potentially more accurate latent semantic representations. 

% Finally, Table \ref{tab:pos_analysis} sheds light on the improvement in the prediction of different parts of speech in the reference summary using the best \texttt{BASS-ADAPT} model. We observe that the proposed model generally improves the prediction of all parts of speech but obtains small improvements on proper nouns. This demonstrates that end-to-end models find named 
% entity prediction challenging, providing a direction for future work. 



% First, we train baseline models on truncated 5-minute and 10-minute long inputs. Then we use BASS to fine-tune the pre-trained 5-minute model on 10 minutes of audio. This is called the block-wise adapted model. We also use BASS to train a model on 10 minutes of audio from scratch and refer to this as the block-wise trained model. 


\begin{table}[!ht]
\caption{Performance of BASS models with block level inference across different implementations of the semantic updater model. Models are pre-trained on 5 minutes and fine-tuned on 10 minutes. R-1, R-2, R-3 represent the ROUGE-1, ROUGE-2, and ROUGE-L metrics respectively}
\label{tab:updater_comparison}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lrrrrr}
    \toprule

Updater    & R-1\uparrow   & R-2\uparrow   & R-L\uparrow   & METEOR\uparrow & BERTScore\uparrow \\ 
\toprule
Concat     & 28.27 & 11.75 & 21.75 & 15.84  & 83.25     \\ 
Gated Attn & 26.15 & 11.22 & 20.49 & 13.80  & 83.52     \\ 
Hier. Attn & 26.11 & 10.50 & 19.50 & 13.30  & 83.40     \\ 
\bottomrule
\end{tabular}
}
\end{table}

\subsection{Comparison of Block-wise Adaptation Strategies}

Table \ref{tab:updater_comparison} compares the various modeling strategies for the semantic updater. We observe that simply concatenating the semantic embedding of the previous (one) block with the current block yields significant improvements in summarization performance. \\




\noindent \textbf{Limitations}: One of the limitations of this work is that BASS requires strong pre-training on truncated inputs to obtain the best performance, along with larger than usual block sizes. For instance, using a few seconds of input for a block is likely insufficient to train a robust model. Attention-based sequence models are not very strong at identifying the correct output lengths ~\cite{deng22b_interspeech}, and this forms another limiting factor in model performance. 



==> sections/setup.tex <==
\subsection{Dataset}
The TEDSummary dataset was introduced by ~\cite{kano2020asru} and expanded with public audio releases in SLUE-TED ~\cite{shon2022slueted}\footnote{The authors of \cite{shon2022slueted} have confirmed that the data will be public}. The data comprises TED talk videos from the TED website\footnote{https://www.ted.com/} until December 2022. The talks are given by renowned speakers from all over the world on very diverse topics, and some talks include multiple speakers. The reference summaries were normalized by converting numbers to their corresponding words and then created by concatenating the title and talk abstract, following ~\cite{kano2020asru,shon2022slueted}. Table \ref{tab:ted_split} highlights the number of videos in the train, validation, and test partitions for the SLUE-TED data.

\begin{table}[!htp]\centering
\caption{SLUE-TED Dataset Statistics} \label{tab:ted_split}
\begin{tabular}{lrr}\toprule
Partition & \#utterances & duration (h)\\\midrule
Train & 3384 & 664\\
Validation & 425 & 81\\
Test & 424 & 84\\
\bottomrule
\end{tabular}
\end{table}



\begin{table*}[!thp]
\centering
\caption{Performance of Block-wise Adaptation and Training Approaches compared to Truncated Baselines with different inference strategies using ROUGE, METEOR, and BERTScore metrics- higher scores indicate better performance}
\label{tab:bass_result_summary}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lllllrrrrr}
\toprule
Training Method & Inference & Pre-training & Train Maxlen & Inf. Maxlen & ROUGE-1\uparrow & ROUGE-2\uparrow & ROUGE-L\uparrow & METEOR\uparrow & BERTScore\uparrow \\ \toprule 
Trunc   & Standard  & X & 5 min & 5 min  & 19.71   & 4.41    & 13.99   & 9.77  & 81.46 \\
Trunc   & Standard  & X & 5 min & 10 min & 20.04  & 4.44    & 14.25   & 9.80   & 81.73 \\ 
\hline  
Trunc  & Standard  & X & 10 min       & 5 min       & 19.18   & 4.23    & 13.52   & 10.21  & 80.75     \\ 
Trunc  & Standard  & X & 10 min       & 10 min      & 19.60    & 4.26    & 13.61   & 10.25  & 80.98     \\  
Trunc ~\cite{shon2022slueted}  & Standard  & X    & 10 min  & Up to 30 mins      &  23.80   & 5.10    & 16.30 & 11.70  & \textbf{84.00}     \\ 
\hline 
BASS-Adapt & Standard  & 5 min & 10 min & 10 min  & \textbf{28.27} & \textbf{11.75} & \textbf{21.75}   & \textbf{15.84} & 83.25     \\ 
BASS-Adapt & Block & 5 min & 10 min & 10 min & 25.48   & 9.48    & 19.10    & 14.27  & 83.17     \\ 
\hline 
BASS-Train & Standard & X & 10 min & 10 min      &    23.01     &    8.18     &  17.19       &  12.10      &  81.60         \\ 
BASS-Train & Block & X & 10 min & 10 min & 26.00    & 11.00    & 20.45   & 13.80  & 83.52     \\ \bottomrule
\end{tabular}
}
\end{table*}

% \subsection{Acoustic Features}
% A key modeling decision is the choice of acoustic features $X$ that can best represent audio for summarization. Traditionally, end-to-end speech models have used spectral Mel-Filterbank (fbank) features, but recent work has shown the benefits of using self-supervised model outputs as input features \cite{sharma2022emotion} for tasks like emotion recognition.   
% In this work, we investigate the difference between these feature representations for the task of speech summarization. We compare the performance of summarization models trained with spectral, WavLM ~\cite{chen2022wavlm} and HuBERT~\cite{hsu2021hubert} features.
% When applying these SSL feature extractors to a downstream task, there is a choice of whether to use only the last layer outputs, or a multi-layer combination of features from different intermediate layers.


%which is a spectrogram representation of the input audio containing frequency information for each timestep. Frequency bins are chosen based on the perceptually linear Mel scale.

% Recent work has also popularized the use of self-supervised learning (SSL) features for speech tasks, such as HuBERT and WavLM . These models are trained on large corpora of unlabeled audio, using auxiliary tasks such as masked input prediction to capture generalizable speech representations.



\subsection{Model Hyperparameters and Evaluation}

\noindent \textbf{Models}: Our models use ESPNet2\footnote{Code will be released to enable reproduction} ~\cite{watanabe2018espnet}  and are first pre-trained on the ASR task using the TED-LIUM 3 \cite{tedlium3} dataset and then fine-tuned on SLUE-TED. The encoder consists of convolutional subsampling by factor 8, followed by 6 conformer \cite{conformer} blocks with 8 attention heads and a hidden size of 1024. The decoder has 6 transformer blocks, with 4 attention heads and a hidden size of 512. The total number of model parameters is 48M. Both the encoder and decoder use a dropout rate of 0.2. We use HuBERT \cite{hsu2021hubert} features as input to the encoder, including a linear preencoder layer to map the features from size 1024 to 80. SpecAugment \cite{specaugment} is used during training and fine-tuning. \\
\noindent \textbf{ASR}: ASR models are trained with Connectionist Temporal Classification (CTC) and Cross-Entropy loss with CTC weight of 0.3. We use the Adam optimizer with peak lr=0.001, and a warmup scheduler for ASR pre-training. This takes 2 days on 8 V-100 32G GPUs

\noindent \textbf{SUMM}: Our summarization models are trained with cross-entropy loss and label smoothing of 0.15. During inference, we use a beam size of 8. Model averaging was not performed as it was found to hurt summarization performance. Fine-tuning is run for a day on one A40 GPU. For BASS models, we use a block size of 15,000 input frames, corresponding to 5 minutes of audio. We only use the semantic embedding from the previous block as context for the current block.

\noindent \textbf{Evaluation}: We evaluate our models with ROUGE \cite{lin-2004-rouge}, METEOR \cite{banerjee-lavie-2005-meteor}, and BERTScore \cite{zhang2020BERTScore}, which are the most common automatic metrics for evaluating summarization models.

==> sections/setup.v2.tex <==
\subsection{Dataset}
The TEDSummary dataset was introduced by ~\cite{kano2020asru} and expanded with public audio releases in SLUE-TED ~\cite{shon2022slueted}\footnote{The authors of \cite{shon2022slueted} have confirmed that the data will be public}. The data comprises TED talk videos from the TED website\footnote{https://www.ted.com/} until December 2022.  The reference summaries were normalized by converting numbers to their corresponding words and then concatenating the title and talk abstract, following ~\cite{kano2020asru,shon2022slueted}. Table \ref{tab:ted_split} highlights the number of videos and length for partitions of SLUE-TED.

%The talks are given by renowned speakers from all over the world on very diverse topics, and some talks include multiple speakers.

\begin{table}[!htp]\centering
\caption{SLUE-TED Dataset Statistics} \label{tab:ted_split}
\begin{tabular}{lrr}\toprule
Partition & \#utterances & duration (h)\\\midrule
Train & 3384 & 664\\
Validation & 425 & 81\\
Test & 424 & 84\\
\bottomrule
\end{tabular}
\end{table}



\begin{table*}[!thp]
\centering
\caption{Performance of Block-wise Adaptation and Training Approaches compared to Truncated Baselines with different inference strategies using ROUGE, METEOR, and BERTScore metrics- higher scores indicate better performance}
\label{tab:bass_result_summary}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lllllrrrrr}
\toprule
Training Method & Inference & Pre-training & Train Maxlen & Inf. Maxlen & ROUGE-1\uparrow & ROUGE-2\uparrow & ROUGE-L\uparrow & METEOR\uparrow & BERTScore\uparrow \\ \toprule 
Trunc   & Standard  & X & 0.5 min & 0.5 min  & 19.71   & 4.41    & 13.99   & 9.77  & 81.46 \\
Trunc   & Standard  & X & 0.5 min & 1 min & 20.04  & 4.44    & 14.25   & 9.80   & 81.73 \\ 
\hline  
Trunc  & Standard  & X & 1 min       & 0.5 min       & 19.18   & 4.23    & 13.52   & 10.21  & 80.75     \\ 
Trunc  & Standard  & X & 1 min       & 1 min      & 19.60    & 4.26    & 13.61   & 10.25  & 80.98     \\  
Trunc ~\cite{shon2022slueted}  & Standard  & X    & 10 min  & Up to 30 mins      &  23.80   & 5.10    & 16.30 & 11.70  & \textbf{84.00}     \\ 
\hline 
BASS-Adapt & Standard  & 0.5 min & 1 min & 1 min  & \textbf{28.27} & \textbf{11.75} & \textbf{21.75}   & \textbf{15.84} & 83.25     \\ 
BASS-Adapt & Block & 0.5 min & 1 min & 1 min & 25.48   & 9.48    & 19.10    & 14.27  & 83.17     \\ 
\hline 
BASS-Train & Standard & X & 1 min & 1 min      &    23.01     &    8.18     &  17.19       &  12.10      &  81.60         \\ 
BASS-Train & Block & X & 1 min & 1 min & 26.00    & 11.00    & 20.45   & 13.80  & 83.52     \\ \bottomrule
\end{tabular}
}
\end{table*}

\subsection{Acoustic Features}
% A key modeling decision is the choice of acoustic features $X$ that can best represent audio for summarization. 
Recent work has shown the benefits of using self-supervised model outputs instead ~\cite{sharma2022emotion} of spectral filterbank features. In this work, we compare spectral, WavLM ~\cite{chen2022wavlm} and HuBERT~\cite{hsu2021hubert} features for summarization.




% When applying these SSL feature extractors to a downstream task, there is a choice of whether to use only the last layer outputs or a multi-layer combination of features from different intermediate layers.


%which is a spectrogram representation of the input audio containing frequency information for each timestep. Frequency bins are chosen based on the perceptually linear Mel scale.

% Recent work has also popularized the use of self-supervised learning (SSL) features for speech tasks, such as HuBERT and WavLM . These models are trained on large corpora of unlabeled audio, using auxiliary tasks such as masked input prediction to capture generalizable speech representations.



\subsection{Model Hyperparameters and Evaluation}

\noindent \textbf{Models}: Our models use ESPNet2\footnote{Code will be released to enable reproduction} ~\cite{watanabe2018espnet}  and are first pre-trained on the ASR task using the TED-LIUM 3 \cite{tedlium3} dataset and then fine-tuned on SLUE-TED. The encoder consists of convolutional subsampling by factor 8, followed by 6 conformer \cite{conformer} blocks with 8 attention heads and a hidden size of 1024. The decoder has 6 transformer blocks, with 4 attention heads and a hidden size of 512. The total number of model parameters is 48M. Both the encoder and decoder use a dropout rate of 0.2. We use HuBERT \cite{hsu2021hubert} features as input to the encoder, including a linear preencoder layer to map the features from size 1024 to 80. SpecAugment \cite{specaugment} is used during training and fine-tuning. \\
\noindent \textbf{ASR}: ASR models are trained with Connectionist Temporal Classification (CTC) and Cross-Entropy loss with a CTC weight of 0.3. We use the Adam optimizer with peak lr=0.001 and a warmup scheduler for ASR pre-training. This takes 2 days on 8 V-100 32G GPUs

\noindent \textbf{SUMM}: Our summarization models are trained with cross-entropy loss and label smoothing of 0.15. During inference, we use a beam size of 8. Model averaging was not performed as it was found to hurt summarization performance. Fine-tuning is run for a day on one A40 GPU. For BASS models, we use a block size of 3,000 input frames, corresponding to 0.5 minutes of audio. We only use the semantic embedding from the previous block as context for the current block.

\noindent \textbf{Evaluation}: We evaluate our models with ROUGE \cite{lin-2004-rouge}, METEOR \cite{banerjee-lavie-2005-meteor}, and BERTScore \cite{zhang2020BERTScore}, which are the most common automatic metrics for evaluating summarization models.
